Delays in Reinforcement Learning

Delays are inherent to most dynamical systems. Besides shifting the process in time, they can significantly affect their performance. For this reason, it is usually valuable to study the delay and account for it. Because they are dynamical systems, it is of no surprise that sequential decision-making problems such as Markov decision processes (MDP) can also be affected by delays. These processes are the foundational framework of reinforcement learning (RL), a paradigm whose goal is to create artificial agents capable of learning to maximise their utility by interacting with their environment. RL has achieved strong, sometimes astonishing, empirical results, but delays are seldom explicitly accounted for. The understanding of the impact of delay on the MDP is limited. In this dissertation, we propose to study the delay in the agent's observation of the state of the environment or in the execution of the agent's actions. We will repeatedly change our point of view on the problem to reveal some of its structure and peculiarities. A wide spectrum of delays will be considered, and potential solutions will be presented. This dissertation also aims to draw links between celebrated frameworks of the RL literature and the one of delays.

==> bibliography.tex <==
\newcommand{\etalchar}[1]{$^{#1}$}
\begin{thebibliography}{AMGW{\etalchar{+}}19}

\bibitem[AA21]{agarwal2021blind}
Mridul Agarwal and Vaneet Aggarwal.
\newblock Blind decision making: Reinforcement learning with delayed observations.
\newblock {\em Pattern Recognition Letters}, 150:176--182, 2021.

\bibitem[ABS99]{altman1999congestion}
Eitan Altman, Tamer Ba{\c{s}}ar, and R~Srikant.
\newblock Congestion control as a stochastic control problem with action delays.
\newblock {\em Automatica}, 35(12):1937--1950, 1999.

\bibitem[ACBF02]{auer2002finite}
Peter Auer, Nicolo Cesa-Bianchi, and Paul Fischer.
\newblock Finite-time analysis of the multiarmed bandit problem.
\newblock {\em Machine learning}, 47(2):235--256, 2002.

\bibitem[AD88]{adke1988limit}
SR~Adke and SR~Deshmukh.
\newblock Limit distribution of a high order markov chain.
\newblock {\em Journal of the Royal Statistical Society: Series B (Methodological)}, 50(1):105--108, 1988.

\bibitem[AHA03]{ait2003stability}
Omar Ait-Hellal and Eitan Altman.
\newblock Stability of abr congestion control using the theory of delayed differential equations.
\newblock {\em International Journal of Systems Science}, 34(10-11):575--584, 2003.

\bibitem[AJO08]{auer2008near}
Peter Auer, Thomas Jaksch, and Ronald Ortner.
\newblock Near-optimal regret bounds for reinforcement learning.
\newblock {\em Advances in neural information processing systems}, 21, 2008.

\bibitem[AKS09]{altman2009stochastic}
Eitan Altman, Vijay Kambley, and Alonso Silva.
\newblock Stochastic games with one step delay sharing information pattern with application to power control.
\newblock In {\em 2009 International Conference on Game Theory for Networks}, pages 124--129. IEEE, 2009.

\bibitem[AMGW{\etalchar{+}}19]{arjona2019rudder}
Jose~A Arjona-Medina, Michael Gillhofer, Michael Widrich, Thomas Unterthiner, Johannes Brandstetter, and Sepp Hochreiter.
\newblock Rudder: Return decomposition for delayed rewards.
\newblock {\em Advances in Neural Information Processing Systems}, 32, 2019.

\bibitem[AN92]{altman1992closed}
Eitan Altman and Philippe Nain.
\newblock Closed-loop control with delayed information.
\newblock {\em ACM sigmetrics performance evaluation review}, 20(1):193--204, 1992.

\bibitem[AO06]{auer2006logarithmic}
Peter Auer and Ronald Ortner.
\newblock Logarithmic online regret bounds for undiscounted reinforcement learning.
\newblock {\em Advances in neural information processing systems}, 19, 2006.

\bibitem[AS73]{alevisakis1973extension}
G~Alevisakis and DE~Seborg.
\newblock An extension of the smith predictor method to multivariable linear systems containing time delays.
\newblock {\em International Journal of Control}, 17(3):541--551, 1973.

\bibitem[ASBB{\etalchar{+}}18]{al-shedivat2018continuous}
Maruan Al-Shedivat, Trapit Bansal, Yura Burda, Ilya Sutskever, Igor Mordatch, and Pieter Abbeel.
\newblock Continuous adaptation via meta-learning in nonstationary and competitive environments.
\newblock In {\em International Conference on Learning Representations (ICLR)}, 2018.

\bibitem[BCB14]{bahdanau2014neural}
Dzmitry Bahdanau, Kyunghyun Cho, and Yoshua Bengio.
\newblock Neural machine translation by jointly learning to align and translate.
\newblock {\em arXiv preprint arXiv:1409.0473}, 2014.

\bibitem[BCDS10]{bayan2010brake}
Fawzi~P Bayan, Anthony~D Cornetto, Ashley Dunn, and Eric Sauer.
\newblock Brake timing measurements for a tractor-semitrailer under emergency braking.
\newblock {\em SAE International Journal of Commercial Vehicles}, 2(2):245--255, 2010.

\bibitem[BCP{\etalchar{+}}16]{brockman2016gym}
Greg Brockman, Vicki Cheung, Ludwig Pettersson, Jonas Schneider, John Schulman, Jie Tang, and Wojciech Zaremba.
\newblock Openai gym, 2016.

\bibitem[Bel54]{bellman1954theory}
Richard Bellman.
\newblock The theory of dynamic programming.
\newblock {\em Bulletin of the American Mathematical Society}, 60(6):503--515, 1954.

\bibitem[Bel66]{bellman1966dynamic}
Richard Bellman.
\newblock Dynamic programming.
\newblock {\em Science}, 153(3731):34--37, 1966.

\bibitem[Ber87]{bertsekas1987dynamic}
Dimitri~P Bertsekas.
\newblock {\em Dynamic Programming: Determinist. and Stochast. Models}.
\newblock Prentice-Hall, 1987.

\bibitem[Ber96]{berchtold1996modelisation}
Andr{\'e} Berchtold.
\newblock Mod{\'e}lisation autor{\'e}gressive des cha{\^\i}nes de markov: Utilisation d'une matrice diff{\'e}rente pour chaque retard.
\newblock {\em Revue de statistique appliqu{\'e}e}, 44(3):5--25, 1996.

\bibitem[BL72]{brooks1972markov}
DM~Brooks and Cornelius~T Leondes.
\newblock Markov decision processes with state-information lag.
\newblock {\em Operations Research}, 20(4):904--907, 1972.

\bibitem[BLS{\etalchar{+}}20]{bisi2020foreign}
Lorenzo Bisi, Pierre Liotet, Luca Sabbioni, Gianmarco Reho, Nico Montali, Marcello Restelli, and Cristiana Corno.
\newblock Foreign exchange trading: A risk-averse batch reinforcement learning approach.
\newblock In {\em Proceedings of the First ACM International Conference on AI in Finance}, pages 1--8, 2020.

\bibitem[Bow74]{bowerman1974nonstationary}
Bruce Bowerman.
\newblock {\em Nonstationary Markov decision processes and related topics in nonstationary Markov chains}.
\newblock PhD thesis, Iowa State University, 1974.

\bibitem[BR02]{berchtold2002mixture}
Andr{\'e} Berchtold and Adrian Raftery.
\newblock The mixture transition distribution model for high-order markov chains and non-gaussian time series.
\newblock {\em Statistical Science}, 17(3):328--356, 2002.

\bibitem[BRB{\etalchar{+}}20]{bouteiller2020reinforcement}
Yann Bouteiller, Simon Ramstedt, Giovanni Beltrame, Christopher Pal, and Jonathan Binas.
\newblock Reinforcement learning with random delays.
\newblock In {\em International Conference on Learning Representations (ICLR)}, 2020.

\bibitem[BS95]{bain1995framework}
Michael Bain and Claude Sammut.
\newblock A framework for behavioural cloning.
\newblock In {\em Machine Intelligence 15}, pages 103--129, 1995.

\bibitem[CBL06]{cesa2006prediction}
Nicolo Cesa-Bianchi and G{\'a}bor Lugosi.
\newblock {\em Prediction, learning, and games}.
\newblock Cambridge university press, 2006.

\bibitem[CCML18]{chua2018deep}
Kurtland Chua, Roberto Calandra, Rowan McAllister, and Sergey Levine.
\newblock Deep reinforcement learning in a handful of trials using probabilistic dynamics models.
\newblock {\em Advances in neural information processing systems}, 31, 2018.

\bibitem[CG16]{chen2016xgboost}
Tianqi Chen and Carlos Guestrin.
\newblock Xgboost: A scalable tree boosting system.
\newblock In {\em Proceedings of the 22nd acm sigkdd international conference on knowledge discovery and data mining}, pages 785--794, 2016.

\bibitem[CGRSS10]{castelletti2010tree}
A~Castelletti, Stefano Galelli, Marcello Restelli, and Rodolfo Soncini-Sessa.
\newblock Tree-based reinforcement learning for optimal water reservoir operation.
\newblock {\em Water Resources Research}, 46(9), 2010.

\bibitem[CGS16]{campbell2016multiple}
Jeffrey~S Campbell, Sidney~N Givigi, and Howard~M Schwartz.
\newblock Multiple model q-learning for stochastic asynchronous rewards.
\newblock {\em Journal of Intelligent \& Robotic Systems}, 81(3):407--422, 2016.

\bibitem[CL18]{chen2018lifelong}
Zhiyuan Chen and Bing Liu.
\newblock Lifelong machine learning.
\newblock {\em Synthesis Lectures on Artificial Intelligence and Machine Learning}, 12(3):1--207, 2018.

\bibitem[CLL95]{chung1995time}
LL~Chung, CC~Lin, and KH~Lu.
\newblock Time-delay control of structures.
\newblock {\em Earthquake Engineering \& Structural Dynamics}, 24(5):687--701, 1995.

\bibitem[CS15]{caarls2015parallel}
Wouter Caarls and Erik Schuitema.
\newblock Parallel online temporal difference learning for motor control.
\newblock {\em IEEE transactions on neural networks and learning systems}, 27(7):1457--1468, 2015.

\bibitem[CT91]{cover1991information}
Thomas~M Cover and Joy~A Thomas.
\newblock Information theory and statistics.
\newblock {\em Elements of information theory}, 1(1):279--335, 1991.

\bibitem[CTS{\etalchar{+}}20]{chandak2020optimizing}
Yash Chandak, Georgios Theocharous, Shiv Shankar, Sridhar Mahadevan, Martha White, and Philip~S Thomas.
\newblock Optimizing for the future in non-stationary mdps.
\newblock {\em ICML 2020}, 2020.

\bibitem[CXLZ21]{chen2021delay}
Baiming Chen, Mengdi Xu, Liang Li, and Ding Zhao.
\newblock Delay-aware model-based reinforcement learning for continuous control.
\newblock {\em Neurocomputing}, 450:119--128, 2021.

\bibitem[CYZ00]{choi2000hidden}
Samuel~PM Choi, Dit-Yan Yeung, and Nevin~L Zhang.
\newblock Hidden-mode markov decision processes for nonstationary sequential decision making.
\newblock In {\em Sequence Learning}, pages 264--287. Springer, 2000.

\bibitem[DCLT18]{devlin2018bert}
Jacob Devlin, Ming-Wei Chang, Kenton Lee, and Kristina Toutanova.
\newblock Bert: Pre-training of deep bidirectional transformers for language understanding.
\newblock {\em arXiv preprint arXiv:1810.04805}, 2018.

\bibitem[DDM21]{derman2021acting}
Esther Derman, Gal Dalal, and Shie Mannor.
\newblock Acting in delayed environments with non-stationary markov policies.
\newblock {\em arXiv preprint arXiv:2101.11992}, 2021.

\bibitem[DFB{\etalchar{+}}22]{degrave2022magnetic}
Jonas Degrave, Federico Felici, Jonas Buchli, Michael Neunert, Brendan Tracey, Francesco Carpanese, Timo Ewalds, Roland Hafner, Abbas Abdolmaleki, Diego de~Las~Casas, et~al.
\newblock Magnetic control of tokamak plasmas through deep reinforcement learning.
\newblock {\em Nature}, 602(7897):414--419, 2022.

\bibitem[DNP13]{deisenroth2013survey}
Marc~Peter Deisenroth, Gerhard Neumann, and Jan Peters.
\newblock A survey on policy search for robotics.
\newblock {\em Foundations and Trends in Robotics}, 2(1-2), 2013.

\bibitem[dSBBE06]{daSilva2006context}
Bruno~C. da~Silva, Eduardo~W. Basso, Ana L.~C. Bazzan, and Paulo~M. Engel.
\newblock Dealing with non-stationary environments using context detection.
\newblock In {\em ICML 2006}, 2006.

\bibitem[DV98]{dugard1998stability}
Luc Dugard and Erik~I Verriest.
\newblock {\em Stability and control of time-delay systems}, volume 228.
\newblock Springer, 1998.

\bibitem[DVDV91]{de1991vernier}
Russell~L De~Valois and Karen~K De~Valois.
\newblock Vernier acuity with stationary moving gabors.
\newblock {\em Vision research}, 31(9):1619--1626, 1991.

\bibitem[EGW05]{ernst2005tree}
Damien Ernst, Pierre Geurts, and Louis Wehenkel.
\newblock Tree-based batch mode reinforcement learning.
\newblock {\em Journal of Machine Learning Research}, 6(Apr):503--556, 2005.

\bibitem[ESM{\etalchar{+}}18]{espeholt2018impala}
Lasse Espeholt, Hubert Soyer, Remi Munos, Karen Simonyan, Vlad Mnih, Tom Ward, Yotam Doron, Vlad Firoiu, Tim Harley, Iain Dunning, et~al.
\newblock Impala: Scalable distributed deep-rl with importance weighted actor-learner architectures.
\newblock In {\em International conference on machine learning}, pages 1407--1416. PMLR, 2018.

\bibitem[FJT18]{firoiu2018human}
Vlad Firoiu, Tina Ju, and Josh Tenenbaum.
\newblock At human speed: Deep reinforcement learning with action delay.
\newblock {\em arXiv preprint arXiv:1810.07286}, 2018.

\bibitem[FLBPP19]{Francois-Lavet2019abstract}
Vincent Francois-Lavet, Yoshua Bengio, Doina Precup, and Joelle Pineau.
\newblock Combined reinforcement learning via abstract representations.
\newblock In {\em AAAI 2019}, 2019.

\bibitem[Fre99]{french1999catastrophic}
Robert~M French.
\newblock Catastrophic forgetting in connectionist networks.
\newblock {\em Trends in cognitive sciences}, 3(4):128--135, 1999.

\bibitem[Fri14]{fridman2014introduction}
Emilia Fridman.
\newblock {\em Introduction to time-delay systems: Analysis and control}.
\newblock Springer, 2014.

\bibitem[G{\etalchar{+}}15]{germain2015made}
Mathieu Germain et~al.
\newblock Made: Masked autoencoder for distribution estimation.
\newblock In {\em International Conference on Machine Learning}, pages 881--889, 2015.

\bibitem[GAACR19]{gong2019decentralized}
Yaobang Gong, Mohamed Abdel-Aty, Qing Cai, and Md~Sharikur Rahman.
\newblock Decentralized network level adaptive signal control by multi-agent deep reinforcement learning.
\newblock {\em Transportation Research Interdisciplinary Perspectives}, 1:100020, 2019.

\bibitem[GBC16]{goodfellow2016deep}
Ian Goodfellow, Yoshua Bengio, and Aaron Courville.
\newblock {\em Deep learning}.
\newblock MIT press, 2016.

\bibitem[GCC{\etalchar{+}}19]{griffiths2019subtasks}
Thomas~L Griffiths, Frederick Callaway, Michael~B Chang, Erin Grant, Paul~M Krueger, and Falk Lieder.
\newblock Doing more with less: meta-reasoning and meta-learning in humans and machines.
\newblock {\em Current Opinion in Behavioral Sciences}, 29:24--30, 2019.
\newblock Artificial Intelligence.

\bibitem[GEW06]{geurts2006extremely}
Pierre Geurts, Damien Ernst, and Louis Wehenkel.
\newblock Extremely randomized trees.
\newblock {\em Machine learning}, 63(1):3--42, 2006.

\bibitem[GN03]{gu2003survey}
Keqin Gu and Silviu-Iulian Niculescu.
\newblock Survey on recent results in the stability and control of time-delay systems.
\newblock {\em J. Dyn. Sys., Meas., Control}, 125(2):158--165, 2003.

\bibitem[GPAM{\etalchar{+}}14]{goodfellow2014generative}
Ian Goodfellow, Jean Pouget-Abadie, Mehdi Mirza, Bing Xu, David Warde-Farley, Sherjil Ozair, Aaron Courville, and Yoshua Bengio.
\newblock Generative adversarial nets.
\newblock {\em Advances in neural information processing systems}, 27, 2014.

\bibitem[GS00]{garcia2000solving}
Alfredo Garcia and Robert~L. Smith.
\newblock Solving nonstationary infinite horizon stochastic production planning problems.
\newblock {\em Oper. Res. Lett.}, 27(3), 2000.

\bibitem[GS13]{ghate2013linear}
Archis Ghate and Robert~L. Smith.
\newblock A linear programming approach to nonstationary infinite-horizon markov decision processes.
\newblock {\em Oper. Res.}, 61(2):413--425, 2013.

\bibitem[Hau00]{hauskrecht2000value}
Milos Hauskrecht.
\newblock Value-function approximations for partially observable markov decision processes.
\newblock {\em Journal of artificial intelligence research}, 13:33--94, 2000.

\bibitem[HBW14]{hadoux2014sequential}
Emmanuel Hadoux, Aur{\'e}lie Beynier, and Paul Weng.
\newblock Sequential decision-making under non-stationary environments via sequential change-point detection.
\newblock In {\em Learning over multiple contexts (LMCE)}, 2014.

\bibitem[HCS{\etalchar{+}}22]{ho2022imagen}
Jonathan Ho, William Chan, Chitwan Saharia, Jay Whang, Ruiqi Gao, Alexey Gritsenko, Diederik~P. Kingma, Ben Poole, Mohammad Norouzi, David~J. Fleet, and Tim Salimans.
\newblock Imagen video: High definition video generation with diffusion models, 2022.

\bibitem[HDCM15]{hallak2015contextual}
Assaf Hallak, Dotan Di~Castro, and Shie Mannor.
\newblock Contextual markov decision processes.
\newblock {\em arXiv preprint arXiv:1502.02259}, 2015.

\bibitem[HHZ{\etalchar{+}}18]{haarnoja2018learning}
Tuomas Haarnoja, Sehoon Ha, Aurick Zhou, Jie Tan, George Tucker, and Sergey Levine.
\newblock Learning to walk via deep reinforcement learning.
\newblock {\em arXiv preprint arXiv:1812.11103}, 2018.

\bibitem[HM82]{hsu1982decentralized}
Kai Hsu and Steven Marcus.
\newblock Decentralized control of finite state markov processes.
\newblock {\em IEEE Transactions on Automatic Control}, 27(2):426--431, 1982.

\bibitem[How60]{howard1960dynamic}
Ronald~A. Howard.
\newblock {\em Dynamic Programming and Markov Processes}.
\newblock MIT Press, Cambridge, MA, 1960.

\bibitem[HPBF21]{howson2021delayed}
Benjamin Howson, Ciara Pike-Burke, and Sarah Filippi.
\newblock Delayed feedback in episodic reinforcement learning.
\newblock {\em arXiv preprint arXiv:2111.07615}, 2021.

\bibitem[HQS12]{hester2012rtmba}
Todd Hester, Michael Quinlan, and Peter Stone.
\newblock Rtmba: A real-time model-based reinforcement learning architecture for robot control.
\newblock In {\em 2012 IEEE International Conference on Robotics and Automation}, pages 85--90. IEEE, 2012.

\bibitem[HRW{\etalchar{+}}22]{han2022off}
Beining Han, Zhizhou Ren, Zuofan Wu, Yuan Zhou, and Jian Peng.
\newblock Off-policy reinforcement learning with delayed rewards.
\newblock In {\em International Conference on Machine Learning}, pages 8280--8303. PMLR, 2022.

\bibitem[HS13]{hester2013texplore}
Todd Hester and Peter Stone.
\newblock Texplore: real-time sample-efficient reinforcement learning for robots.
\newblock {\em Machine learning}, 90(3):385--429, 2013.

\bibitem[HSU12]{hachiya2012importance}
Hirotaka Hachiya, Masashi Sugiyama, and Naonori Ueda.
\newblock Importance-weighted least-squares probabilistic classifier for covariate shift adaptation with application to human activity recognition.
\newblock {\em Neurocomputing}, 80:93--101, 2012.

\bibitem[HY18]{hannah2018unbounded}
Robert Hannah and Wotao Yin.
\newblock On unbounded delays in asynchronous parallel fixed-point algorithms.
\newblock {\em Journal of Scientific Computing}, 76(1):299--326, 2018.

\bibitem[HZAL18]{haarnoja2018soft}
Tuomas Haarnoja, Aurick Zhou, Pieter Abbeel, and Sergey Levine.
\newblock Soft actor-critic: Off-policy maximum entropy deep reinforcement learning with a stochastic actor.
\newblock In {\em International conference on machine learning}, pages 1861--1870. PMLR, 2018.

\bibitem[Jac88]{jacobson1988congestion}
Van Jacobson.
\newblock Congestion avoidance and control.
\newblock {\em ACM SIGCOMM computer communication review}, 18(4):314--329, 1988.

\bibitem[JBKS15]{jain2015comparative}
Aditya Jain, Ramta Bansal, Avnish Kumar, and KD~Singh.
\newblock A comparative study of visual and auditory reaction times on the basis of gender and physical activity levels of medical first year students.
\newblock {\em International Journal of Applied and Basic Medical Research}, 5(2):124, 2015.

\bibitem[JGS13]{joulani2013online}
Pooria Joulani, Andras Gyorgy, and Csaba Szepesv{\'a}ri.
\newblock Online learning under delayed feedback.
\newblock In {\em International Conference on Machine Learning}, pages 1453--1461. PMLR, 2013.

\bibitem[JMC{\etalchar{+}}17]{jaderberg2017rew-pred}
Max Jaderberg, Volodymyr Mnih, Wojciech~Marian Czarnecki, Tom Schaul, Joel~Z. Leibo, David Silver, and Koray Kavukcuoglu.
\newblock Reinforcement learning with unsupervised auxiliary tasks.
\newblock In {\em International Conference on Learning Representations (ICLR)}, 2017.

\bibitem[JMdR19]{jagerman2019people}
Rolf Jagerman, Ilya Markov, and Maarten de~Rijke.
\newblock When people change their mind: Off-policy evaluation in non-stationary recommendation environments.
\newblock In {\em Proceedings of the Twelfth ACM International Conference on Web Search and Data Mining}, pages 447--455, 2019.

\bibitem[KD18]{kingma2018glow}
Durk~P Kingma and Prafulla Dhariwal.
\newblock Glow: Generative flow with invertible 1x1 convolutions.
\newblock {\em Advances in neural information processing systems}, 31, 2018.

\bibitem[KE03]{katsikopoulos2003markov}
Konstantinos~V Katsikopoulos and Sascha~E Engelbrecht.
\newblock Markov decision processes with delays and asynchronous cost collection.
\newblock {\em IEEE transactions on automatic control}, 48(4):568--574, 2003.

\bibitem[KKLM03]{kwon2003simple}
Wook~Hyun Kwon, Jin~Won Kang, Young~Sam Lee, and Young~Soo Moon.
\newblock A simple receding horizon control for state delayed systems and its stability criterion.
\newblock {\em Journal of Process Control}, 13(6):539--551, 2003.

\bibitem[KL02]{kakade2002approximately}
Sham Kakade and John Langford.
\newblock Approximately optimal approximate reinforcement learning.
\newblock In {\em In Proc. 19th International Conference on Machine Learning}. Citeseer, 2002.

\bibitem[KLC98]{kaelbling1998planning}
Leslie~Pack Kaelbling, Michael~L Littman, and Anthony~R Cassandra.
\newblock Planning and acting in partially observable stochastic domains.
\newblock {\em Artificial intelligence}, 101(1-2):99--134, 1998.

\bibitem[KNG99]{kolmanovskii1999delay}
Vladimir~B Kolmanovskii, S-I Niculescu, and Keqin Gu.
\newblock Delay effects on stability: A survey.
\newblock In {\em Proceedings of the 38th IEEE Conference on Decision and Control (Cat. No. 99CH36304)}, volume~2, pages 1993--1998. IEEE, 1999.

\bibitem[KRRP20]{khetarpal2020towards}
Khimya Khetarpal, Matthew Riemer, Irina Rish, and Doina Precup.
\newblock Towards continual reinforcement learning: A review and perspectives.
\newblock {\em arXiv preprint arXiv:2012.13490}, 2020.

\bibitem[KSH17]{krizhevsky2017imagenet}
Alex Krizhevsky, Ilya Sutskever, and Geoffrey~E Hinton.
\newblock Imagenet classification with deep convolutional neural networks.
\newblock {\em Communications of the ACM}, 60(6):84--90, 2017.

\bibitem[KST{\etalchar{+}}21]{kiran2021deep}
B~Ravi Kiran, Ibrahim Sobh, Victor Talpaert, Patrick Mannion, Ahmad~A Al~Sallab, Senthil Yogamani, and Patrick P{\'e}rez.
\newblock Deep reinforcement learning for autonomous driving: A survey.
\newblock {\em IEEE Transactions on Intelligent Transportation Systems}, 2021.

\bibitem[KV15]{kumar2015stochastic}
Panqanamala~Ramana Kumar and Pravin Varaiya.
\newblock {\em Stochastic systems: Estimation, identification, and adaptive control}.
\newblock SIAM, 2015.

\bibitem[LAL{\etalchar{+}}20]{liotet2020deep}
P~Liotet, Patrice Abry, R~Leonarduzzi, Marc Senneret, Laurent Jaffres, and Gerald Perrin.
\newblock Deep learning abilities to classify intricate variations in temporal dynamics of multivariate time series.
\newblock In {\em ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, pages 3857--3861. IEEE, 2020.

\bibitem[LB08]{lebre2008algorithm}
Sophie L{\`e}bre and Pierre-Yves Bourguignon.
\newblock An em algorithm for estimation in the mixture transition distribution model.
\newblock {\em Journal of Statistical Computation and Simulation}, 78(8):713--729, 2008.

\bibitem[LCB22]{laroche2022non}
Romain Laroche, Remi Tachet~des Combes, and Jacob Buckman.
\newblock Non-markovian policies occupancy measures.
\newblock {\em arXiv preprint arXiv:2205.13950}, 2022.

\bibitem[Lew14]{lewis2014flash}
Michael Lewis.
\newblock {\em Flash boys: a Wall Street revolt}.
\newblock WW Norton \& Company, 2014.

\bibitem[LHP{\etalchar{+}}16]{lillicrap2015continuous}
Timothy~P. Lillicrap, Jonathan~J. Hunt, Alexander Pritzel, Nicolas Heess, Tom Erez, Yuval Tassa, David Silver, and Daan Wierstra.
\newblock Continuous control with deep reinforcement learning.
\newblock In Yoshua Bengio and Yann LeCun, editors, {\em International Conference on Learning Representations (ICLR)}, 2016.

\bibitem[LLF{\etalchar{+}}17]{laskey2017dart}
Michael Laskey, Jonathan Lee, Roy Fox, Anca Dragan, and Ken Goldberg.
\newblock Dart: Noise injection for robust imitation learning.
\newblock In {\em Conference on robot learning}, pages 143--156. PMLR, 2017.

\bibitem[LMBR22]{liotet2022delayed}
Pierre Liotet, Davide Maran, Lorenzo Bisi, and Marcello Restelli.
\newblock Delayed reinforcement learning by imitation.
\newblock In Kamalika Chaudhuri, Stefanie Jegelka, Le~Song, Csaba Szepesvari, Gang Niu, and Sivan Sabato, editors, {\em Proceedings of the 39th International Conference on Machine Learning}, volume 162 of {\em Proceedings of Machine Learning Research}, pages 13528--13556. PMLR, 17--23 Jul 2022.

\bibitem[LP17]{levin2017markov}
David~A Levin and Yuval Peres.
\newblock {\em Markov chains and mixing times}, volume 107.
\newblock American Mathematical Soc., 2017.

\bibitem[LR19]{lecarpentier2019non}
Erwan Lecarpentier and Emmanuel Rachelson.
\newblock Non-stationary markov decision processes, a worst-case approach using model-based reinforcement learning.
\newblock {\em Advances in neural information processing systems}, 32, 2019.

\bibitem[LS98]{loch1998using}
John Loch and Satinder Singh.
\newblock Using eligibility traces to find the best memoryless policy in partially observable markov decision processes.
\newblock In {\em ICML}, volume~98, pages 323--331, 1998.

\bibitem[LS15]{lesner2015nonstationary}
Boris Lesner and Bruno Scherrer.
\newblock Non-stationary approximate modified policy iteration.
\newblock In Francis~R. Bach and David~M. Blei, editors, {\em ICML 2015}, 2015.

\bibitem[LS20]{lattimore2020bandit}
Tor Lattimore and Csaba Szepesv{\'a}ri.
\newblock {\em Bandit algorithms}.
\newblock Cambridge University Press, 2020.

\bibitem[LSKM21]{lancewicki2021stochastic}
Tal Lancewicki, Shahar Segal, Tomer Koren, and Yishay Mansour.
\newblock Stochastic multi-armed bandits with unrestricted delay distributions.
\newblock In {\em International Conference on Machine Learning}, pages 5969--5978. PMLR, 2021.

\bibitem[LVMR22]{liotet2022lifelong}
Pierre Liotet, Francesco Vidaich, Alberto~Maria Metelli, and Marcello Restelli.
\newblock Lifelong hyper-policy optimization with multiple importance sampling regularization.
\newblock In {\em Proceedings of the AAAI Conference on Artificial Intelligence}, 2022.

\bibitem[LVR21]{liotet2021learning}
Pierre Liotet, Erick Venneri, and Marcello Restelli.
\newblock Learning a belief representation for delayed reinforcement learning.
\newblock In {\em 2021 International Joint Conference on Neural Networks (IJCNN)}, pages 1--8. IEEE, 2021.

\bibitem[MBM{\etalchar{+}}16]{mnih2016asynchronous}
Volodymyr Mnih, Adria~Puigdomenech Badia, Mehdi Mirza, Alex Graves, Timothy Lillicrap, Tim Harley, David Silver, and Koray Kavukcuoglu.
\newblock Asynchronous methods for deep reinforcement learning.
\newblock In {\em International conference on machine learning}, pages 1928--1937. PMLR, 2016.

\bibitem[MC89]{mccloskey1989catastrophic}
Michael McCloskey and Neal~J Cohen.
\newblock Catastrophic interference in connectionist networks: The sequential learning problem.
\newblock In {\em Psychology of learning and motivation}, volume~24, pages 109--165. Elsevier, 1989.

\bibitem[MGY{\etalchar{+}}21]{mirhoseini2021graph}
Azalia Mirhoseini, Anna Goldie, Mustafa Yazgan, Joe~Wenjie Jiang, Ebrahim Songhori, Shen Wang, Young-Joon Lee, Eric Johnson, Omkar Pathak, Azade Nazi, et~al.
\newblock A graph placement methodology for fast chip design.
\newblock {\em Nature}, 594(7862):207--212, 2021.

\bibitem[MKKB18]{mahmood2018setting}
A~Rupam Mahmood, Dmytro Korenkevych, Brent~J Komer, and James Bergstra.
\newblock Setting up a reinforcement learning task with a real-world robot.
\newblock In {\em 2018 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)}, pages 4635--4640. IEEE, 2018.

\bibitem[MKS{\etalchar{+}}13]{mnih2013playing}
Volodymyr Mnih, Koray Kavukcuoglu, David Silver, Alex Graves, Ioannis Antonoglou, Daan Wierstra, and Martin Riedmiller.
\newblock Playing atari with deep reinforcement learning.
\newblock {\em arXiv preprint arXiv:1312.5602}, 2013.

\bibitem[MMB{\etalchar{+}}20]{metelli2020control}
Alberto~Maria Metelli, Flavio Mazzolini, Lorenzo Bisi, Luca Sabbioni, and Marcello Restelli.
\newblock Control frequency adaptation via action persistence in batch reinforcement learning.
\newblock In {\em International Conference on Machine Learning}, pages 6862--6873. PMLR, 2020.

\bibitem[MMMS21]{mysore2021regularizing}
Siddharth Mysore, Bassel Mabsout, Renato Mancuso, and Kate Saenko.
\newblock Regularizing action policies for smooth control with reinforcement learning.
\newblock In {\em 2021 IEEE International Conference on Robotics and Automation (ICRA)}, pages 1810--1816. IEEE, 2021.

\bibitem[MPFR18]{metelli2018policy}
Alberto~Maria Metelli, Matteo Papini, Francesco Faccio, and Marcello Restelli.
\newblock Policy optimization via importance sampling.
\newblock In {\em NeurIPS 2018}, 2018.

\bibitem[MPMR20]{metelli2020importance}
Alberto~Maria Metelli, Matteo Papini, Nico Montali, and Marcello Restelli.
\newblock Importance sampling techniques for policy optimization.
\newblock {\em Journal of Machine Learning Research}, 21(141):1--75, 2020.

\bibitem[MVHS14]{mahmood2014weighted}
A~Rupam Mahmood, Hado~P Van~Hasselt, and Richard~S Sutton.
\newblock Weighted importance sampling for off-policy learning with linear function approximation.
\newblock {\em Advances in Neural Information Processing Systems}, 27, 2014.

\bibitem[MWE20]{mendez2020lifelong}
Jorge Mendez, Boyu Wang, and Eric Eaton.
\newblock Lifelong policy gradient learning of factored policies for faster training without forgetting.
\newblock {\em Advances in Neural Information Processing Systems}, 33:14398--14409, 2020.

\bibitem[MZY22]{mao2022active}
Yiqian Mao, Shan Zhong, and Hujun Yin.
\newblock Active flow control using deep reinforcement learning with time delays in markov decision process and autoregressive policy.
\newblock {\em Physics of Fluids}, 34(5):053602, 2022.

\bibitem[Nic01]{niculescu2001delay}
Silviu-Iulian Niculescu.
\newblock {\em Delay effects on stability: a robust control approach}, volume 269.
\newblock Springer Science \& Business Media, 2001.

\bibitem[Nij94]{nijhawan1994motion}
Romi Nijhawan.
\newblock Motion extrapolation in catching.
\newblock {\em Nature}, 1994.

\bibitem[NMT10]{nayyar2010optimal}
Ashutosh Nayyar, Aditya Mahajan, and Demosthenis Teneketzis.
\newblock Optimal control strategies in delayed sharing information structures.
\newblock {\em IEEE Transactions on Automatic Control}, 56(7):1606--1620, 2010.

\bibitem[NT20]{nota2020policy}
Chris Nota and Philip~S Thomas.
\newblock Is the policy gradient a gradient?
\newblock In {\em Proceedings of the 19th International Conference on Autonomous Agents and MultiAgent Systems}, pages 939--947, 2020.

\bibitem[ODZ{\etalchar{+}}16]{oord2016wavenet}
Aaron van~den Oord, Sander Dieleman, Heiga Zen, Karen Simonyan, Oriol Vinyals, Alex Graves, Nal Kalchbrenner, Andrew Senior, and Koray Kavukcuoglu.
\newblock Wavenet: A generative model for raw audio.
\newblock {\em arXiv preprint arXiv:1609.03499}, 2016.

\bibitem[OGA20]{ortner2020uclr2}
Ronald Ortner, Pratik Gajane, and Peter Auer.
\newblock Variational regret bounds for reinforcement learning.
\newblock In {\em UAI 2020}, 2020.

\bibitem[OPN18]{osa2018algorithmic}
Takayuki Osa, Joni Pajarinen, and Gerhard Neumann.
\newblock {\em An Algorithmic Perspective on Imitation Learning}.
\newblock Now Publishers Inc., Hanover, MA, USA, 2018.

\bibitem[Owe13]{mcbook}
Art~B. Owen.
\newblock {\em Monte Carlo theory, methods and examples}.
\newblock 2013.

\bibitem[Pad21]{padakandla2021survey}
Sindhu Padakandla.
\newblock A survey of reinforcement learning algorithms for dynamically varying environments.
\newblock {\em ACM Computing Surveys (CSUR)}, 54(6):1--25, 2021.

\bibitem[PBASG18]{pike2018bandits}
Ciara Pike-Burke, Shipra Agrawal, Csaba Szepesvari, and Steffen Grunewalder.
\newblock Bandits with delayed, aggregated anonymous feedback.
\newblock In {\em International Conference on Machine Learning}, pages 4105--4113. PMLR, 2018.

\bibitem[PMLR19]{papini2019optimistic}
Matteo Papini, Alberto~Maria Metelli, Lorenzo Lupo, and Marcello Restelli.
\newblock Optimistic policy optimization via multiple importance sampling.
\newblock In {\em ICML 2019}, 2019.

\bibitem[PPM17]{papamakarios2017masked}
George Papamakarios, Theo Pavlakou, and Iain Murray.
\newblock Masked autoregressive flow for density estimation.
\newblock In I.~Guyon, U.~Von Luxburg, S.~Bengio, H.~Wallach, R.~Fergus, S.~Vishwanathan, and R.~Garnett, editors, {\em Advances in Neural Information Processing Systems}, volume~30. Curran Associates, Inc., 2017.

\bibitem[PS08]{peters2008reinforcement}
Jan Peters and Stefan Schaal.
\newblock Reinforcement learning of motor skills with policy gradients.
\newblock {\em Neural networks}, 21(4):682--697, 2008.

\bibitem[PT87]{papadimitriou1987complexity}
Christos~H Papadimitriou and John~N Tsitsiklis.
\newblock The complexity of markov decision processes.
\newblock {\em Mathematics of operations research}, 12(3):441--450, 1987.

\bibitem[PTR21]{poiani2021meta}
Riccardo Poiani, Andrea Tirinzoni, and Marcello Restelli.
\newblock Meta-reinforcement learning by tracking task non-stationarity.
\newblock In {\em {IJCAI}}, pages 2899--2905. ijcai.org, 2021.

\bibitem[Put94]{puterman1994markov}
Martin~L Puterman.
\newblock Markov decision processes: Discrete stochastic dynamic programming, 1994.

\bibitem[R{\etalchar{+}}61]{renyi1961measures}
Alfr{\'e}d R{\'e}nyi et~al.
\newblock On measures of entropy and information.
\newblock In {\em Proceedings of the fourth Berkeley symposium on mathematical statistics and probability}, volume~1, pages 547--561. Berkeley, California, USA, 1961.

\bibitem[Raf85a]{raftery1985model}
Adrian~E Raftery.
\newblock A model for high-order markov chains.
\newblock {\em Journal of the Royal Statistical Society: Series B (Methodological)}, 47(3):528--539, 1985.

\bibitem[Raf85b]{raftery1985new}
AE~Raftery.
\newblock A new model for discrete-valued time series: autocorrelations and extensions.
\newblock {\em Rassegna di Metodi Statistici ed Applicazioni}, 3(4):149--162, 1985.

\bibitem[RAT{\etalchar{+}}22]{romano2022multi}
Giulia Romano, Andrea Agostini, Francesco Trov{\`o}, Nicola Gatti, and Marcello Restelli.
\newblock Multi-armed bandit problem with temporally-partitioned rewards: When partial feedback counts.
\newblock In Lud~De Raedt, editor, {\em Proceedings of the Thirty-First International Joint Conference on Artificial Intelligence, {IJCAI-22}}, pages 3401--3407. International Joint Conferences on Artificial Intelligence Organization, 7 2022.
\newblock Main Track.

\bibitem[RB10]{ross2010efficient}
St{\'e}phane Ross and Drew Bagnell.
\newblock Efficient reductions for imitation learning.
\newblock In {\em Proceedings of the thirteenth international conference on artificial intelligence and statistics}, pages 661--668. JMLR Workshop and Conference Proceedings, 2010.

\bibitem[RBL{\etalchar{+}}21a]{riva2021learning}
Antonio Riva, Lorenzo Bisi, Pierre Liotet, Luca Sabbioni, Edoardo Vittori, Marco Pinciroli, Michele Trapletti, and Marcello Restelli.
\newblock Learning fx trading strategies with fqi and persistent actions.
\newblock In {\em Proceedings of the Second ACM International Conference on AI in Finance}, pages 1--9, 2021.

\bibitem[RBL{\etalchar{+}}21b]{rombach2021highresolution}
Robin Rombach, Andreas Blattmann, Dominik Lorenz, Patrick Esser, and Björn Ommer.
\newblock High-resolution image synthesis with latent diffusion models, 2021.

\bibitem[RBL{\etalchar{+}}22]{riva2022addressing}
Antonio Riva, Lorenzo Bisi, Pierre Liotet, Luca Sabbioni, Edoardo Vittori, Marco Pinciroli, Michele Trapletti, and Marcello Restelli.
\newblock Addressing non-stationarity in fx trading with online model selection of offline rl experts.
\newblock 2022.

\bibitem[RCA{\etalchar{+}}19]{riemer2018learning}
Matthew Riemer, Ignacio Cases, Robert Ajemian, Miao Liu, Irina Rish, Yuhai Tu, and Gerald Tesauro.
\newblock Learning to learn without forgetting by maximizing transfer and minimizing interference.
\newblock In {\em In International Conference on Learning Representations (ICLR)}, 2019.

\bibitem[RDN{\etalchar{+}}22]{ramesh2022hierarchical}
Aditya Ramesh, Prafulla Dhariwal, Alex Nichol, Casey Chu, and Mark Chen.
\newblock Hierarchical text-conditional image generation with clip latents.
\newblock {\em arXiv preprint arXiv:2204.06125}, 2022.

\bibitem[RGB11]{ross2011reduction}
St{\'e}phane Ross, Geoffrey Gordon, and Drew Bagnell.
\newblock A reduction of imitation learning and structured prediction to no-regret online learning.
\newblock In {\em Proceedings of the fourteenth international conference on artificial intelligence and statistics}, pages 627--635. JMLR Workshop and Conference Proceedings, 2011.

\bibitem[Ric03]{richard2003time}
Jean-Pierre Richard.
\newblock Time-delay systems: an overview of some recent advances and open problems.
\newblock {\em automatica}, 39(10):1667--1694, 2003.

\bibitem[RL10]{rachelson2010locality}
E.~Rachelson and M.~G. Lagoudakis.
\newblock {O}n the {L}ocality of {A}ction {D}omination in {S}equential {D}ecision {M}aking.
\newblock In {\em Tenth Intl. Symposium on AI and Math}, 2010.

\bibitem[RM15]{rezende2015variational}
Danilo Rezende and Shakir Mohamed.
\newblock Variational inference with normalizing flows.
\newblock In {\em Proceedings of the 32nd International Conference on Machine Learning}, volume~37 of {\em Proceedings of Machine Learning Research}, pages 1530--1538. PMLR, 2015.

\bibitem[RN94]{rummery1994line}
Gavin~A Rummery and Mahesan Niranjan.
\newblock {\em On-line Q-learning using connectionist systems}, volume~37.
\newblock Citeseer, 1994.

\bibitem[RP19]{ramstedt2019real}
Simon Ramstedt and Chris Pal.
\newblock Real-time reinforcement learning.
\newblock {\em Advances in neural information processing systems}, 32, 2019.

\bibitem[RRT21]{ren2021applying}
Feng Ren, Jean Rabault, and Hui Tang.
\newblock Applying deep reinforcement learning to active flow control in weakly turbulent conditions.
\newblock {\em Physics of Fluids}, 33(3):037121, 2021.

\bibitem[SB18]{sutton2018reinforcement}
Richard~S Sutton and Andrew~G Barto.
\newblock {\em Reinforcement learning: An introduction}.
\newblock MIT press, 2018.

\bibitem[SBBJ10]{schuitema2010control}
Erik Schuitema, Lucian Bu{\c{s}}oniu, Robert Babu{\v{s}}ka, and Pieter Jonker.
\newblock Control delay in reinforcement learning for real-time dynamic systems: a memoryless approach.
\newblock In {\em 2010 IEEE/RSJ International Conference on Intelligent Robots and Systems}, pages 3226--3231. IEEE, 2010.

\bibitem[SCS{\etalchar{+}}22]{saharia2022photorealistic}
Chitwan Saharia, William Chan, Saurabh Saxena, Lala Li, Jay Whang, Emily Denton, Seyed Kamyar~Seyed Ghasemipour, Burcu~Karagol Ayan, S~Sara Mahdavi, Rapha~Gontijo Lopes, et~al.
\newblock Photorealistic text-to-image diffusion models with deep language understanding.
\newblock {\em arXiv preprint arXiv:2205.11487}, 2022.

\bibitem[SHM{\etalchar{+}}16]{silver2016mastering}
David Silver, Aja Huang, Chris~J Maddison, Arthur Guez, Laurent Sifre, George Van Den~Driessche, Julian Schrittwieser, Ioannis Antonoglou, Veda Panneershelvam, Marc Lanctot, et~al.
\newblock Mastering the game of go with deep neural networks and tree search.
\newblock {\em nature}, 529(7587):484--489, 2016.

\bibitem[SLA{\etalchar{+}}15]{schulman2015trust}
John Schulman, Sergey Levine, Pieter Abbeel, Michael Jordan, and Philipp Moritz.
\newblock Trust region policy optimization.
\newblock In {\em International conference on machine learning}, pages 1889--1897. PMLR, 2015.

\bibitem[SMAD17]{Shelhamer2017dyn-pred}
Evan Shelhamer, Parsa Mahmoudieh, Max Argus, and Trevor Darrell.
\newblock Loss is its own reward: Self-supervision for reinforcement learning.
\newblock In {\em International Conference on Learning Representations (ICLR)}, 2017.

\bibitem[Smi57]{smith1957closer}
Otto~JM Smith.
\newblock Closer control of loops with dead time.
\newblock {\em Chemical engineering progress}, 53:217--219, 1957.

\bibitem[SMSM99]{sutton1999policy}
Richard~S Sutton, David McAllester, Satinder Singh, and Yishay Mansour.
\newblock Policy gradient methods for reinforcement learning with function approximation.
\newblock {\em Advances in neural information processing systems}, 12, 1999.

\bibitem[SOR{\etalchar{+}}08]{sehnke2008parameter}
Frank Sehnke, Christian Osendorfer, Thomas R{\"{u}}ckstie{\ss}, Alex Graves, Jan Peters, and J{\"{u}}rgen Schmidhuber.
\newblock Policy gradients with parameter-based exploration for control.
\newblock In Vera Kurkov{\'{a}}, Roman Neruda, and Jan Koutn{\'{\i}}k, editors, {\em ICANN 2008}, 2008.

\bibitem[Spa12]{spaan2012partially}
Matthijs~TJ Spaan.
\newblock Partially observable markov decision processes.
\newblock In {\em Reinforcement Learning}, pages 387--414. Springer, 2012.

\bibitem[SPH{\etalchar{+}}22]{singer2022make}
Uriel Singer, Adam Polyak, Thomas Hayes, Xi~Yin, Jie An, Songyang Zhang, Qiyuan Hu, Harry Yang, Oron Ashual, Oran Gafni, et~al.
\newblock Make-a-video: Text-to-video generation without text-video data.
\newblock {\em arXiv preprint arXiv:2209.14792}, 2022.

\bibitem[SPS99]{sutton1999between}
Richard~S Sutton, Doina Precup, and Satinder Singh.
\newblock Between mdps and semi-mdps: A framework for temporal abstraction in reinforcement learning.
\newblock {\em Artificial intelligence}, 112(1-2):181--211, 1999.

\bibitem[SWD{\etalchar{+}}17]{schulman2017proximal}
John Schulman, Filip Wolski, Prafulla Dhariwal, Alec Radford, and Oleg Klimov.
\newblock Proximal policy optimization algorithms.
\newblock {\em CoRR}, abs/1707.06347, 2017.

\bibitem[TET12]{todorov2012mujoco}
Emanuel Todorov, Tom Erez, and Yuval Tassa.
\newblock Mujoco: A physics engine for model-based control.
\newblock In {\em 2012 IEEE/RSJ International Conference on Intelligent Robots and Systems}, pages 5026--5033. IEEE, 2012.

\bibitem[TMSP18]{travnik2018reactive}
Jaden~B Travnik, Kory~W Mathewson, Richard~S Sutton, and Patrick~M Pilarski.
\newblock Reactive reinforcement learning in asynchronous environments.
\newblock {\em Frontiers in Robotics and AI}, 5:79, 2018.

\bibitem[TS09]{taylor2009transfer}
Matthew~E Taylor and Peter Stone.
\newblock Transfer learning for reinforcement learning domains: A survey.
\newblock {\em Journal of Machine Learning Research}, 10(7), 2009.

\bibitem[TSPR18]{pmlr-v80-tirinzoni18a}
Andrea Tirinzoni, Andrea Sessa, Matteo Pirotta, and Marcello Restelli.
\newblock Importance weighted transfer of samples in reinforcement learning.
\newblock In {\em ICML 2018}, 2018.

\bibitem[U{\etalchar{+}}16]{uria2016neural}
Benigno Uria et~al.
\newblock Neural autoregressive distribution estimation.
\newblock {\em The Journal of Machine Learning Research}, 17(1):7184--7220, 2016.

\bibitem[VBC{\etalchar{+}}19]{vinyals2019grandmaster}
Oriol Vinyals, Igor Babuschkin, Wojciech~M Czarnecki, Micha{\"e}l Mathieu, Andrew Dudzik, Junyoung Chung, David~H Choi, Richard Powell, Timo Ewalds, Petko Georgiev, et~al.
\newblock Grandmaster level in starcraft ii using multi-agent reinforcement learning.
\newblock {\em Nature}, 575(7782):350--354, 2019.

\bibitem[VEH14]{van2014renyi}
Tim Van~Erven and Peter Harremos.
\newblock R{\'e}nyi divergence and kullback-leibler divergence.
\newblock {\em IEEE Transactions on Information Theory}, 60(7):3797--3820, 2014.

\bibitem[VG95]{veach1995monte}
Eric Veach and Leonidas~J. Guibas.
\newblock Optimally combining sampling techniques for monte carlo rendering.
\newblock In Susan~G. Mair and Robert Cook, editors, {\em SIGGRAPH 1995}, 1995.

\bibitem[Vil09]{villani2009optimal}
C{\'e}dric Villani.
\newblock {\em Optimal transport: old and new}, volume 338.
\newblock Springer, 2009.

\bibitem[VSP{\etalchar{+}}17]{vaswani2017attention}
Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones, Aidan~N Gomez, {\L}ukasz Kaiser, and Illia Polosukhin.
\newblock Attention is all you need.
\newblock {\em Advances in neural information processing systems}, 30, 2017.

\bibitem[VW78]{varaiya1978delayed}
Pravin Varaiya and Jean Walrand.
\newblock On delayed sharing patterns.
\newblock {\em IEEE Transactions on Automatic Control}, 23(3):443--445, 1978.

\bibitem[W{\etalchar{+}}09]{walsh2009learning}
Thomas~J Walsh et~al.
\newblock Learning and planning in environments with delayed feedback.
\newblock {\em Autonomous Agents and Multi-Agent Systems}, 18(1):83, 2009.

\bibitem[Wat89]{watkins1989learning}
C.~J. C.~H. Watkins.
\newblock {\em Learning from Delayed Rewards}.
\newblock PhD thesis, King's College, Oxford, 1989.

\bibitem[WC17]{wu2017markov}
Sheng-Jhih Wu and Moody~T Chu.
\newblock Markov chains with memory, tensor formulation, and the dynamics of power iteration.
\newblock {\em Applied Mathematics and Computation}, 303:226--239, 2017.

\bibitem[WD92]{watkins1992q}
Christopher~JCH Watkins and Peter Dayan.
\newblock Q-learning.
\newblock {\em Machine learning}, 8:279--292, 1992.

\bibitem[Wil92]{williams1992simple}
Ronald~J Williams.
\newblock Simple statistical gradient-following algorithms for connectionist reinforcement learning.
\newblock {\em Mach Learn}, 8(3):229--256, 1992.

\bibitem[Wil93]{wilcox1993effect}
Jarrod~W Wilcox.
\newblock The effect of transaction costs and delay on performance drag.
\newblock {\em Financial Analysts Journal}, 49(2):45--54, 1993.

\bibitem[Wit71]{witsenhausen1971separation}
Hans~S Witsenhausen.
\newblock Separation of estimation and control for discrete time systems.
\newblock {\em Proceedings of the IEEE}, 59(11):1557--1566, 1971.

\bibitem[XJK{\etalchar{+}}20]{xiao2020thinking}
Ted Xiao, Eric Jang, Dmitry Kalashnikov, Sergey Levine, Julian Ibarz, Karol Hausman, and Alexander Herzog.
\newblock Thinking {While} {Moving}: Deep {Reinforcement} {Learning} with {Concurrent} {Control}.
\newblock {\em International Conference on Learning Representations (ICLR)}, 2020.

\bibitem[XLY20]{xu2020error}
Tian Xu, Ziniu Li, and Yang Yu.
\newblock Error bounds of imitating policies and environments.
\newblock {\em Advances in Neural Information Processing Systems}, 33, 2020.

\bibitem[ZSP18]{zhang2018decoupling}
Amy Zhang, Harsh Satija, and Joelle Pineau.
\newblock Decoupling dynamics and reward for transfer learning.
\newblock In {\em ICLR (workshop) 2018}, 2018.

\end{thebibliography}


==> chapters/acknowledge.tex <==
Acknowledgements.


==> chapters/summary.tex <==
\chapter*{Summary}
\lettrine{S}{ummary} goes here.

